TaxThemis: Interactive Mining and Exploration of Suspicious Tax Evasion Group

Tax evasion is a serious economic problem for many countries, as it can undermine the government' s tax system and lead to an unfair business competition environment. Recent research has applied data analytics techniques to analyze and detect tax evasion behaviors of individual taxpayers. However, they failed to support the analysis and exploration of the uprising related party transaction tax evasion (RPTTE) behaviors (e.g., transfer pricing), where a group of taxpayers is involved. In this paper, we present TaxThemis, an interactive visual analytics system to help tax officers mine and explore suspicious tax evasion groups through analyzing heterogeneous tax-related data. A taxpayer network is constructed and fused with the trade network to detect suspicious RPTTE groups. Rich visualizations are designed to facilitate the exploration and investigation of suspicious transactions between related taxpayers with profit and topological data analysis. Specifically, we propose a calendar heatmap with a carefully-designed encoding scheme to intuitively show the evidence of transferring revenue through related party transactions. We demonstrate the usefulness and effectiveness of TaxThemis through two case studies on real-world tax-related data, and interviews with domain experts.

==> archive/1-intro-archive.tex <==
\firstsection{Introduction}
% \maketitle

% 1. Introduce the background and importance of detecting suspicious tax evasion group. Specifically, we need to emphasize the importance of detecting suspicious tax evasion group. You can refer to the introduction part of the 5 papers in the ``related work/tax'' folder. Then, we briefly discuss the data we have, which makes the data-driven detection of suspicious tax evasion group possible. 

% the severe tax evasion problem and its influence
% Tax Evasion is an illegal activities of taxpayers declaring less profits or overstating costs to evade tax. The Joint Committee on Taxation (JCT) proposed tax gap, the difference between tax liability and tax paid on time to measure the influence of tax evasion~\cite{mazur_understanding_2007}. The severe tax evasion problem has resulted serious tax gap of government worldwide.
% The definition of tax evasion and tax gap
Tax evasion is a severe financial crime against the tax system in which taxpayers deliberately report false financial position to deny their tax obligations. It is one of the most significant factors in the tax gap, that is the difference between the tax revenue a government is entitled to receive and actually received. 
%For instance, the estimated tax gap was amounted to 441 billion USD per year for the 2011-2013 period in the United States~\cite{irs_2019}.
%Also in Europe, the estimated value-added tax gap are over 147 billion Euros in 2016 ~\cite{poniatowski_study_2018}.
%In Italy, it is estimated about 97 billion Euros tax gap each year in 2013-2015 period~\cite{didimo_combining_2020}.
%And in the United Kingdom, the tax gap is estimated amounted to 33 billion in 2016-2017~\cite{HM_2018}.
% This gives the monetary value of the impact
In the United Kingdom, the size of the tax gap was estimated at £35 billion in 2017/18~\cite{HM_2019}.
% This gives the ratio to GDP which more people understands
Alongside the predicted tax gap for 28 European Union countries were, on average, 7.7\% of their GDP in 2015.~\cite{global_tax_gap_2018}.
%The severe tax gap also occurs in developing country. 
%It was reported that the average tax loss rate was over 26\% in China according to the calculation by the end of 20th century~\cite{chengcorrelation}.
% This describes social and economic impacts other than tax revenue
Besides less government revenue for civil service budgets, a severe tax gap has other economic and social implications, such as eroding the profitability of self-compliant taxpayers over dishonest competitors and inciting more non-compliance to exploit the vulnerable tax system~\cite{oecd_2017}.

% Lots of efforts have been put into handling the tax evasion issues by tax administrations all over the world.
In light of the enormous impacts, tax authorities have spent tremendous human and time efforts in scrutinizing tax evasion behaviors.
% For example, 
% Without the popularity of electronic invoice, 
Traditional tax inspection has mainly focused on detecting individual tax evasion behaviors such as account manipulations, and fake invoices~\cite{tian_mining_2016}.
% \noindent However, there comes a new tendency of group-based tax evasion behavior\cite{tian_mining_2016}\cite{ruan_identifying_2019}. 
Some recent approaches target at investigating group-based tax evasion behaviors~\cite{tian_mining_2016,ruan_identifying_2019}.
The goal of these methods is to identify a group of related taxpayers who attempted to conceal the real revenue and cost to avoid tax by making false invoices or transfer pricing. Such kind of taxpayer groups are often called \textit{Affiliated Transaction Based Tax Evasion (ATTE)} group~\cite{ruan_identifying_2019}.
% It refers to a group of related taxpayers revealing the real revenue or cost to reduce tax  by making false invoice or transfer pricing, which is called affiliated transaction based tax evasion(ATTE) group.
It is estimated by the Organization for Economic Cooperation and Development (OECD) estimated that the tax gap caused by ATTE is 4 to 10 percent of the total tax revenue from corporate profit tax worldwide by 2016~\cite{tselykh_attributed_2016}. 


% Major tax inspection ways
Since the group-based tax evasion behavior is well organized by a group of taxpayers with real trading record. Both the detection difficulty and impact have aroused great attention of tax authorities~\cite{davia_accountants_2000}. To detect it, there are three major ways in daily tax inspection including: manual case selection~\cite{wu_using_2012}, whistle-blowing selection~\cite{bowen_whistle-blowing_2010}, and computer-based selection ~\cite{wu_using_2012,liu_application_2010}. 
Since the amount of taxpayers is far more than the amount of tax inspectors, it is preferred to use computer-based methods to detect such tax evasion groups~\cite{wu_using_2012,tian_mining_2016}.
The advanced computer-based techniques can generally be categorized into two types: machine learning method~\cite{tian_mining_2016,tselykh_attributed_2016,abou-nasr_data_2015,kim_detecting_2016,lee_fuzzy_2010} and graph-based method~\cite{tselykh_attributed_2016,tian_mining_2016}.

% machine learning based method
Machine learning method focus on dividing taxpayers into tax evasion or not based on their individual characteristics. More specifically, such method can be categorized as association analysis~\cite{matos_empirical_2014,chen_delphi-based_2010}, cluster analysis~\cite{czarnowski_detecting_2016,castellon_gonzalez_characterization_2013}, and classification method~\cite{chen_delphi-based_2010}. 
% limitation of machine learning method
Although they have achieved high accuracy in detecting tax evasion, the result is hard to be understand by tax inspectors since they don't offer the specific reason to be identified.

% graph-based method
Different from machine learning method, graph-based methods focus on structure characteristics of tax evasion groups. They generating a pattern tree based on structure characteristics of tax evasion cases, and applying a pattern matching algorithm into a constructed heterogeneous taxpayer interest interacted network(TPIIN) to detect suspicious tax evasion group~\cite{tian_mining_2016,ruan_identifying_2019,tselykh_attributed_2016}.
% limitation of graph-based method
However, they neither consider the link attribute(such as link weight) nor in view of the node attribute(such as financial indices and evasion record) in each group, resulting in high false positives rate. 
% Also, not considering indirect affiliated transaction caused high false negatives rate.

% the large amount of suspicious groups brings new difficulty for tax inspectors to identify, while they are not concerned about checking other related abnormal factors of taxpayers such as financial indexes, historical product price, and tax evasion record.


% 2. Discuss the challenges of detecting suspicious tax evasion group (for example, the big size of the data, the intrinsically heterogeneous data properties, etc. ). Meanwhile, you may also briefly discuss the major limitations of existing approaches (e.g., those automated algorithms). 

% the limitation of 
\noindent The limitations of existing work come from three aspects. 
(1) Machine learning based methods is less reliable since they do not offer the specific reason of their classification results for detecting a tax evader. Also, both the intrinsically heterogeneous tax data properties and the large amount of their classification result brings difficulty to and further exploring the specific tax evasion evidence to identify their results .
(2) Graph-based method not consider integrating the association strength(how strength they are associated) and related individual characteristics(such as financial statement, audit log),
caused high false positive rate.
% The association strength is proposed to evaluate how strength they are associated and calculated by integrating the amount of link, link step and link attribute (invest rate value) between the related taxpayers. 
(3) None of them considers the indirect trading behavior between related party, caused missing identification of potential tax evasion group, and resulting high false negative rate.


% (1) Machine learning based method and graph-based method only focus either the individual characteristic or the structure characteristics, caused high false positive rate. That means, a large amount of suspicious groups requires extra effort of tax inspectors to be verified. 
% (2) The intrinsically heterogeneous tax data properties brings difficulty to explore the specific tax evasion evidence to identify each suspicious group.
% (3) None of them integrating association strength between related taxpayers and the indirect trading between related parties to help tax administrations inspect the potential tax evasion behaviors.
% (1) The amount of suspicious group detected from the graph-based method is too large, which requires extra effort on verify each suspicious group.
% (2) The result of the machine learning method is hard to interpret without offering tax evasion evidence.
% (3) The intrinsically heterogeneous data properties brings difficulty to check the origin data of each group.
% (4) They either focus on related parties or focus on affiliated transactions. 
% None of them considers integrating related strength and the historical insidious transactions between related parties to help tax administrations inspect the potential tax evasion behaviors.

% To tackle the above issues, our corporate tax authorities offer us the origin tax data to support deeper research on detecting tax evasion groups, which makes the data-driven detection of suspicious tax evasion groups possible.
% Our data is collected from the financial statement, register information of taxpayers,and invoice data between taxpayers from 2014 to 2015 in a province from China. 
% Because of data confidentiality, we desensitize the origin data. The final available data consists of the taxpayer data, trade data, investment data, and auditing record. 




% 3. Introduce our work and briefly discuss how our approach will handle the challenges discussed above.

Inspired by the successful works combining visual analytic techniques and data mining algorithm in analyzing financial frauds~\cite{dilla_data_2015,kielman_foundations_2009,leite_visual_2018}, we use visual analytic technique combining the data mining algorithm to overcome the above limitations of existing works in group-based tax evasion detection.

Our data mining algorithm is adapted from~\cite{tian_mining_2016}, which can quickly analyze the data and effectively identify the high risky tax evasion taxpayer groups. The workflow of the algorithm is as follows. First, they use a graph-based method to extract the characteristic of affiliated transaction from classical tax evasion cases. Then, they construct a Taxpayer Interest Interacted Network(TPIIN) based on a colored network-based model to depict the interest relationships between taxpayers, such as trading, invest and legal representative. Finally, they detect the suspicious tax evasion groups based on a pattern matching algorithm by building the patterns tree and the pattern matching component of tax evasion group.

% Visual analytic techniques, combined with data mining algorithms, have recently proved their effectiveness and advantages in analyzing financial frauds~\cite{dilla_data_2015,kielman_foundations_2009,leite_visual_2018}.
% Inspired by these studies, 
To further analyse those suspicious tax evasion group and overcome the limitation of existing works, we present {\name}, a visual analytic system to help tax inspectors explore and identify suspicious tax evasion groups. 
We work closely with a local tax administration office in China for 3 years to understand the detailed requirements of tax evasion detection and iteratively refine our system. All the data used in this paper, including the taxpayer information, auditing logs, trade and investment records, are all from our collaboration tax administration office after conducting data masking on the original data.
% First, we apply the data mining algorithm to get the set of suspicious tax evasion groups since their approach can narrow down a list of suspicious groups. 


The proposed visual analytics system consists of three major views: the overview, the filter view, the graph view, and the detail view. 

The overview visualize all the suspicious tax evasion groups detected by algorithm adapted from~\cite{tian_mining_2016} with a T-SNE design to help users quickly explore and identify suspicious tax evasion groups with similar features. The feature of each group including the number of taxpayers in the group, the total assets of the group, the association strength of the affiliated transaction in the group, and the total affiliated transaction amount in the group. In addition, we encode the suspect value and influence value as node opacity and size in this view to help users explore by interest.
The filter view visualizes the tax evasion risk indices of a list of suspicious tax evasion  groups
% These suspicious tax evasion groups are detected by the algorithm adapted from~\cite{tian_mining_2016}
, which can help tax inpector quickly analyze the data and effectively identify the high risky tax evasion groups.
Users can interactively change those metrics to filter possible tax evasion groups of their interest. The metrics include a time slider for choosing a time period of interest affiliated transaction, and a maximum link length of interest.
% Next, we offer a filter view, propose several indices to quantify a suspect value and an influence value of the affiliated transaction in each group and support interactive filtering by those quantified indices. This view makes the large amount of suspicious groups accessible and evaluable. 
The graph view shows the detailed relationship structure of the tax evasion group, where each node of the graph is a novel glyph that encodes the basic taxpayer information such as capital, industry and tax indices.
% Then, A graph view with novel glyph design and encoding scheme is proposed to show the detailed relationship structure in a focused group with encoding their basic taxpayer data.
% The relationship structure in the graph view shows why they are considered as suspicious group. 
In particular, we encode the evasion record and indirect relationship as context to support evidence discovering. 
% Since the anomaly information, including related strength and the historical insidious transactions, is encoded in graph view, the tax evasion evidence can be easily explored and identified. 
Users can easily explore and confirm the exact tax evasion groups through viewing and checking the association strength and historical insidious transactions from color encoding and link width encoding of the graph view. 
% Also, the origin multivariate data of each taxpayer will be shown in a detailed view to support exploration and knowledge discovery. The intrinsically heterogeneous data properties can be intuitively demonstrated based on the data type.
The detail view shows the intrinsically heterogeneous data of focused taxpayer, including the monthly financial indices, establish time, major merchandise, and industry of a selected taxpayer to support exploration and knowledge discovery.

% Last but not least, we extract the features of each suspicious group to plot a TSNE view and encode its suspect value and influence value. This view is shown to facilitate users to batch processing suspicious groups. That means, it enables tax inspectors to explore suspicious groups with similar features with current identified tax evasion groups.
% To further help users quickly explore and identify suspicious tax evasion groups that may be not detected by our algorithm, we design the T-SNE view to visualize the similarity of different companies or their legal representatives, which can help tax inspectors to quickly identify suspicious groups that have similar features with current confirmed tax evasion group.
We evaluated {\name} through two case studies and carefully-designed interviews with domain experts, which demonstrates its effectiveness and usability in helping tax inspectors to quickly and confidently explore and identify tax evasion groups.



% 4. Briefly discuss the evaluations (case studies and expert interviews) and list the major contributions of our approach:

% - A interactive visual analytics system for detecting tax evasion group.

% - Any novel designs?

% - Case studies on real world dataset and interviews with tax administrator. 

% \noindent Furthermore, we evaluate the effectiveness of TaxLens through three case studies and expert interviews. 


Our contributions can be summarized as follows:
\begin{itemize}
  \item We propose an interactive visual analytics system, {\name}, to enable the quick exploration, detection, and identification of tax evasion groups.
  \item We present a set of novel visual designs to facilitate the ranking, inspection, and perception of most suspect tax evasion groups in real tax dataset. Specifically, we propose a novel glyph to encode the profile information of taxpayers and abnormal indexes. Also, a new focus+context approach based visual design is used to show the historical indirect transactions between taxpayers, which help the tax inspector with further identification.
  \item We conduct two case studies with the real tax dataset and held well-structured expert interviews with xx 
  local tax administration officials in China, which demonstrate the effectiveness and usefulness of {\name}.
  
  
%   A usage scenario with a realworld tax dataset and three case studies with expert interviews with  tax inspectors that demonstrate the effectiveness and usefulness of {\name}.

\end{itemize}






